Affective Translation: Material and Virtual Embodiments of Kinetic Textile Robots

This study presents a comparative framework for evaluating emotional engagement with textile soft robots and their augmented-reality (AR) counterparts. Four robotic sculptures were developed, each embodying nature-inspired dynamic behaviors such as breathing and gradual deformation. Using a between-subjects design, two independent groups, one experiencing the physical installations and one engaging with their virtual (AR) twins, follow identical protocols and complete the same self-assessment survey on affective and perceptual responses. This approach minimizes carryover and novelty effects while enabling a direct comparison of sensations such as calmness, curiosity, and discomfort across modalities. The analysis explores how motion, form, and material behavior shape emotional interpretation in physical versus digital contexts, informing the design of hybrid systems that evoke meaningful, emotionally legible interactions between humans, robots, and digital twins.

==> data/methodology.tex <==
\textbf{3. Methodology} 

\textbf{3.1 Overview} 

This study examines how people emotionally and perceptually respond to textile soft robots across physical and virtual embodiments. Both systems initially share the same geometry and motion sequence. After this baseline comparison. This allows us to undestand how the emotional resposnses alter between interacting with a real life soft robot vs interact with it in the ar envoriment. 

\textbf{3.2 Building of the physical pieces} 

\textbf{3.2.1 Physical System Design} 

The physical textile soft robots were developed through an iterative process that bridges material experimentation, color theory, and mechanical design. Each piece in the \textit{Sympathetic Motion} series was conceived as a living system composed of three interdependent layers  muscle, skeleton, and skin that together define the sculpture’s movement, material behavior, and perceived personality. 

\textbf{3.2.1.1Actuation systems  }

 The internal “muscles” are networks of flexible strings, pneumatic chambers, and mechanical elements that expand and contract through controlled air pressure or linear actuation. These actuation systems were designed to evoke rhythms found in living organisms  breathing, pulsing, and swelling rather than mechanical repetition. The movement patterns were refined through cycles of coding, video observation, and manual testing to achieve motions that feel soft, delayed, and slightly unpredictable qualities that audiences interpret as alive. 

\textbf{3.2.1.2 Structural elements }

The supporting structure, or “skeleton,” combines lightweight materials such as wood, 3D-printed joints, and soft fillers that act as internal “fat.” These elements define the sculpture’s form and guide its deformation during motion. Each configuration was carefully tuned so the kinetic transformation could emerge smoothly, balancing rigidity with compliance. The resulting forms are semi-collapsible, allowing for surprise transitions and easy transport  a practical benefit discovered through iterative prototyping. 

\textbf{3.2.1.3 Surface Design }

The outermost layer  the “skin”  is where material, pattern, and perception meet. Working first in white muslin similarly used in fashion allows one read the form purely through its movement before introducing surface design. Once the behavior of a piece feels coherent, custom-printed fabrics are developed to alter how the audience perceives that same motion. Most of the fabrics used are 90 \% poly spandex and are printed via Heatpress method. 

Across prototypes, three main strategies were tested for surface–form interaction: 

Independent patterning — surface prints that disregard the object’s seams, causing the pattern to distort as the sculpture moves. This technique often conceals construction lines and produces a surprisingly lifelike quality. 

Contour-aligned patterning — patterns that trace the object’s sewn geometry, emphasizing edges and amplifying its volumetric presence. 

Interrupted patterning — hybrid surfaces where pattern fades intermittently into solid color, revealing underlying form only in fragments. This partial concealment produces an effect of unpredictability, as if the object were intermittently revealing itself. 

Different methods create a unique emotional tone. In other series, we have experimented with various ways of designing patterns. For this series, the printed imagery comes from multiple sources: photographs of underwater organisms, traced and recolored natural patterns, and vectorized designs for digital fabric prints. 

In \textit{Waiting for the Dark}, these design principles converge. The sculpture’s patterned spandex skin follows the curvature of its soft body while contrasting translucent blues and reds create what Josef Albers called \textit{vibrating boundary} zones where complementary colors produce optical flicker. For some viewers, this effect reads as alive or pulsating; for others, it feels disorienting or “scary.” This chromatic tension becomes a perceptual equivalent of breath: attraction and resistance intertwined. 

Each prototype’s fabrication required iterative calibration between material resistance and motion rhythm. Sewing techniques, internal pocket placement, and actuator routing were adjusted to control airflow and deformation. Every finished sculpture thus embodies a negotiation between mechanical logic and sensory affect a textile organism designed not to imitate life but to evoke it through motion, texture, and surface resonance. 

